Perceptions of Moderators as a Large-Scale Measure of Online Community Governance

Millions of online communities are governed by volunteer moderators, who shape their communities by setting and enforcing rules, recruiting additional moderators, and participating in the community themselves. These moderators must regularly make decisions about how to govern, yet measuring the 'success' of governance is complex and nuanced, making it challenging to determine what governance strategies are most successful. Furthermore, prior work has shown that communities have differing values, suggesting that 'one-size-fits-all' approaches to governance are unlikely to serve all communities well. In this work, we assess governance practices on reddit by classifying the sentiment of community members' public discussion of their own moderators. We label 1.89 million posts and comments made on reddit over an 18 month period. We relate these perceptions to characteristics of community governance, and to different actions that community moderators take. We identify types of communities where moderators are perceived particularly positively and negatively, and highlight promising strategies for moderator teams. Amongst other findings, we show that strict rule enforcement is linked to more favorable perceptions of moderators of communities dedicated to certain topics, such as news communities, than others. We investigate what kinds of moderators are associated with improved community perceptions upon their addition to a mod team, and find that moderators who are active community members before and during their mod tenures are seen more favorably. We make our models, anonymized datasets, and code public.

==> 07_checklist.tex <==
\subsection{Required Paper Checklist}

%  README
% For each question, change the default Answer to Yes, and,
% No, because, or NA, when the question seems inappropriate
% for your research study. You are strongly encouraged to in-
% clude a justification to your answer, either by referencing
% the appropriate section of your paper or providing a brief in-
% line description. Within the Checklist section, you may sup-
% plement your answers with a brief discussion that expands
% on answers to the checklist where necessary.

% For example:
% - Did you include the license to the code and datasets? Yes,
% see the Methods and the Appendix
% - Did you include the license to the code and datasets? No,
% because the code and the data are proprietary.
% - Did you include the license to the code and datasets? NA

% see here for more: https://www.overleaf.com/project/64f2930710fcd91b3045d354

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Impacts from the research are discussed in \sect\ref{sec:intro} and \ref{sec:discussion}, ethical and privacy concerns are discussed in \sect\ref{sec:ethics}.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, discussed in \sect\ref{sec:methods}.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, discussed in \sect\ref{sec:limitations}.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, see \sect\ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, discussed in \sect\ref{sec:limitations}.}
  \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, discussed in \sect\ref{sec:ethics}.}
  \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, described in \sect\ref{sec:ethics}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{Not applicable.}
  \item Have you provided justifications for all theoretical results?
    \answerNA{Not applicable.}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{Not applicable.}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerYes{Yes, discussed in \sect\ref{sec:rq1}, \ref{sec:rq2} and \ref{sec:limitations}.}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerYes{Yes, addresed in \sect\ref{sec:rq1}, \ref{sec:rq2} and \ref{sec:limitations}.}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerYes{Yes, see \sect\ref{sec:related}.}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerYes{Yes, discussed in \sect\ref{sec:intro}, \ref{sec:rq1}, \ref{sec:rq2}, and \ref{sec:discussion}.}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{Not applicable.}
  \item Did you include complete proofs of all theoretical results?
    \answerNA{Not applicable.}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, complete details and code for training models and reproducing results will be included with our codebase which will be made public upon publication.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, complete details and code for training models and reproducing results will be included with our codebase which will be made public upon publication.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, bootstrapped CIs are included in every figure.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, detailed in \sect\ref{sec:outcomes}.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, discussed throughout \sect\ref{sec:rq1} and \ref{sec:rq2}, and addressed specifically in \sect\ref{sec:limitations}.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerYes{Yes, discussed in \sect\ref{sec:rq1}, \ref{sec:rq2} and \ref{sec:limitations}.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, cited in \sect\ref{sec:related} and \ref{sec:methods}.}
  \item Did you mention the license of the assets?
    \answerYes{Yes, in \sect\ref{sec:ethics}.}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerYes{A dataset sample is included in the supplemental material, and our full code, models, and datasets will be made public upon publication.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes, discussed in \sect\ref{sec:ethics}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Yes, in \sect\ref{sec:ethics} and in Appendix~\ref{app:additional_figs}.}
  \item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
    \answerYes{Yes, in \sect\ref{sec:ethics} and in Appendix~\ref{app:additional_figs}.}  
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
    \answerYes{Yes, in \sect\ref{sec:ethics} and in Appendix~\ref{app:additional_figs}.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{Not applicable.}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{Not applicable.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Not applicable.}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNA{Not applicable.}
\end{enumerate}

\end{enumerate}
